SciFact-Open: Towards open-domain scientific claim verification

While research on scientific claim verification has led to the development of powerful systems that appear to approach human performance, these approaches have yet to be tested in a realistic setting against large corpora of scientific literature. Moving to this open-domain evaluation setting, however, poses unique challenges; in particular, it is infeasible to exhaustively annotate all evidence documents. In this work, we present SciFact-Open, a new test collection designed to evaluate the performance of scientific claim verification systems on a corpus of 500K research abstracts. Drawing upon pooling techniques from information retrieval, we collect evidence for scientific claims by pooling and annotating the top predictions of four state-of-the-art scientific claim verification models. We find that systems developed on smaller corpora struggle to generalize to SciFact-Open, exhibiting performance drops of at least 15 F1. In addition, analysis of the evidence in SciFact-Open reveals interesting phenomena likely to appear when claim verification systems are deployed in practice, e.g., cases where the evidence supports only a special case of the claim. Our dataset is available at https://github.com/dwadden/scifact-open.

==> fig/_old/gold_recall_wrapper.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{fig/gold_recall.pdf}

  \caption{
      Recall of gold evidence. The upper bound is the fraction of gold evidence that was retrieved.
  } 
  \label{fig:gold_recall}
\end{figure}


==> fig/label_confusion_wrapper.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{fig/label_confusion.pdf}
  \caption{TODO}
  \label{fig:label_confusion}
\end{figure}


==> sec_conclusion.tex <==
\section{Conclusion}

In this work, we introduce the task of open-domain scientific claim verification and release a novel test set, \scifactOpen, to support performance evaluation for this task. Given the large and ever-changing set of scientific articles that make up the evidence corpora for scientific claims, models must be able to scale and adapt accordingly. Our findings suggest that current state-of-the-art systems do not generalize well to this more realistic task variant. It is our hope that the dataset and analyses presented in this work will facilitate future modeling improvements, and lead to substantial gains in our understanding of the scientific claim verification task.  


==> sec_introduction_alternative.tex <==
\section{Introduction}

The task of scientific claim verification aims to assess the veracity of a scientific claim relative to a textual context~\cite{Wadden2020FactOF}. Most existing work and available datasets focus on verifying claims against a fairly narrow context, such as a single article or text snippet \cite{Saakyan2021COVIDFactFE,Sarrouti2021EvidencebasedFO,Kotonya2020ExplainableAF}, or a small, artificially-constructed corpus \cite{Wadden2020FactOF}. However, it is important to verify scientific claims against a large body of scientific research since the the literature is constantly expanding, as is the number of online corpora on which a fact verification system might be deployed.

While some recent work explores verifying claims against a large-scale scientific corpus, it evaluates systems on their accuracy at predicting a single global truth label \cite{Stammbach2021TheCO}. However, the corpus may  contain \emph{conflicting evidence}: some documents may \support the claim, while others may \refute it. Moreover, the \emph{weight} of the evidence --- i.e. the total number of documents supporting and refuting the claim --- is a crucial factor in making decisions about the likely truth of scientific claims.  Meanwhile, exhaustive  annotation of claims and evidences  is infeasible for large corpora, a challenge frequently encountered in Information Retrieval (IR)~\cite{xx}.
%This context could be as specific as a single sentence from a scientific article~\cite{xxx}, or a  as general as the corpus of all abstracts in PubMed. When the context is a single sentence, scientific claim verification can be framed as an NLI task, and accomplished by predicting whether the context sentence \supports, \refutes, or is neutral with respect to the claim. 

In this work, we study \emph{open-domain scientific claim verification}, framed and evaluated as identifying and labeling all documents which \support and / or \refute a given claim with respect to a large-scale corpus of documents. We are motivated by two research questions. First, are models trained to verify claims against a limited context (e.g. a small corpus) able to generalize to much larger corpora not seen during training, and can we reliably compare the generalization performance of different models in this setting? % The ability to characterize model behavior under this kind of distribution shift is particularly important for scientific claim verification, since the body of scientific evidence is constantly expanding, as is the number of online corpora on which a fact verification system might be deployed. 
Second, does open fact verification present novel NLP challenges that were less apparent in a more restricted context?
%Motivated by real-world applications (cite something here), scientific claim verification is best framed and evaluated as identifying and labeling all documents which \support and / or \refute the claim. 


\input{fig/teaser_wrapper.tex}



% TODO I'm here.

To make progress on these questions, we present \scifactOpen,  a new test set for open-domain scientific claim verification where original claims and evidences are taken from \scifact dataset \cite{Wadden2020FactOF} (which we call \scifactOrig) and new evidences are collected   from a corpus of 500K scientific research abstracts. We use a \emph{pooling} strategy (popularized by the TREC competitions~\cite{xx}) that uses a collection of existing fact verification models~\cite{ss} to identify likely evidences for claim, and then collects human annotations for the candidate evidences. Section \ref{sec:data} discusses our choices of fact-checking models,  the criteria used to prioritize candidate evidences for annotation, and the number of candidates to annotate. Our  experiments  confirm that the collected annotations are extensive enough to facilitate reliable model evaluation.

Using our newly-collected dataset, we find that generalization to the open-domain setting represents a substantial challenge for existing fact verification models, and that the best-performing model on \scifactOrig was over-fit to the abstracts in the original dataset. In addition, we find that conflicting evidence is fairly common in \scifactOpen, and is often caused by claim ambiguity: cases where one special case of the input claim is supported by evidence is refuted, and a different special case is refuted. We are optimistic that our new dataset, analysis, and suggested ``best practices'' for studying open-domain scientific claim verification will motivate future work on this relevant and challenging task.

% To make progress on these questions, we construct a new test set for open-domain scientific claim verification, which we call \scifactOpen. \scifactOpen uses the same claims as the original \scifact test set \cite{Wadden2020FactOF} (referred to as \scifactOrig), and verifies them against a corpus of 500K abstracts from the \storc corpus \cite{Lo2020S2ORCTS}; this represents a hundred-fold increase over the size of the \scifactOrig corpus. 

% Each claim in \scifactOpen is paired with a set of \emph{evidence abstracts} --- i.e. abstracts from the corpus containing evidence which \supports or \refutes the claim. These evidence abstracts are obtained from two sources. First, we include all evidence from \scifactOrig. Second, we collect new evidence from the \scifactOpen corpus using a data collection strategy known as \emph{pooling}: we use four state-of-the-art models developed for the original \scifact task to predict evidence candidates from \scifactOpen, and then manually annotate the predicted candidates. 



%%%%%%%%%%%%%%%%%%%%


% Motivated by the spread of scientific mis- and dis-information online, the NLP research community has made substantial progress on the task of verifying biomedical claims against evidence found in research literature, including the release of scientific claim verification datasets and the development of novel modeling approaches.

% However, there is a mismatch between the settings in which this task has been studied, and the setting in which we would hope to deploy scientific claim verification systems. Existing scientific claim verification datasets either provide the evidence necessary to verify a given claim as a task input \cite{Saakyan2021COVIDFactFE,Sarrouti2021EvidencebasedFO}, or else require the model to retrieve evidence from a small, carefully-constructed corpus containing a few thousand documents \cite{Wadden2020FactOF}. By contrast, we would like to use these systems to verify claims against large bodies of scientific evidence --- for instance, all abstracts available on PubMed. We refer to this setting as \emph{open-domain scientific claim verification}.




% While recent results suggest that existing models can achieve near human-level performance in these restricted settings \cite{Wadden2021MultiVerSIS}, there is no test set available to evaluate the performance of science fact-checking models in the more realistic setting where they must retrieve evidence from a scientific corpus containing hundreds of thousands of documents.

% To address this challenge, we present \scifactOpen, an expanded version of the \scifact test set where claims are verified against a corpus of 500K documents sampled from the \storc dataset \cite{Lo2020S2ORCTS}. This represents a hundred-fold increase over the size of the original \scifact corpus. Since manually annotating each document \dave{Since manually annotating each claim / evidence pair} in the corpus for evidence is not feasible, we follow a data collection strategy popularized by the TREC competitions \cite{Voorhees1999OverviewOT,Voorhees1998OverviewOT} known as \emph{pooling}: use four state-of-the-art claim verification systems to identify documents likely to contain evidence, annotate the 250 most-confident predictions from each model, and perform computational checks to confirm that the number of annotations collected (known as the \emph{pool depth}) is sufficient to facilitate reliable evaluation on new models \cite{Zobel1998HowRA}. This annotation process leads to the identification of 311 \dave{This number is wrong.} additional claim / evidence pairs, which we combine with the 209 pairs from the original \scifact test set to constitute \scifactOpen.


% % TODO make this better.
% We find that \scifactOpen is challenging for state-of-the-art scientific claim verification models, which achieve performance roughly 50 F1 (compared to 70 F1 on the original dataset). In addition, we find that the strongest-performing system on \scifact was over-fit to the documents in the original \scifact corpus, and that model generalization behavior is heavily dependent on the the negative sampling rate used during training. We are optimistic that \scifactOpen will facilitate the development of modeling approaches and the identification of new challenges and sub-tasks for open-domain scientific claim verification.


==> sec_introduction_old.tex <==
\section{Introduction}

% NOTE this version was too verbose; I've made a new one.

The task of scientific claim verification aims to assess the veracity of a scientific claim relative to a textual context. This context could be as specific as a single sentence from a scientific article, or as general as the corpus of all abstracts in PubMed. When the context is a single sentence, scientific claim verification can be framed as an NLI task, and accomplished by predicting whether the context sentence \supports, \refutes, or is neutral with respect to the claim. 

By contrast, when the context is a large body of scientific research, predicting a single ``global'' truth label indicating the relationship between claim and evidence as a whole is inappropriate, for two reasons (see Fig. \ref{fig:teaser} for an example). First, the corpus may contain \emph{conflicting evidence}: some documents may \support the claim, while others may \refute it. Second, the \emph{weight} of the evidence --- i.e. the total number of documents supporting and refuting the claim --- is a crucial factor in making decisions about the likely truth of scientific claims. 

Therefore, claim verification against a large body of evidence is best framed and evaluated as an information retrieval task, where the goal is to identify and label all documents which \support and / or \refute the claim. This is the most realistic and compelling use case for scientific claim verification systems. However, evaluating model predictions in this setting presents a challenge frequently encountered in IR: exhaustive relevance annotation (annotating whether every document in the corpus \supports or \refutes each claim in the dataset) is infeasible for large corpora. 

Due to this challenge, most existing work and available datasets focus on verifying claims against a fairly narrow context, such as a single article or text snippet \cite{Saakyan2021COVIDFactFE,Sarrouti2021EvidencebasedFO,Kotonya2020ExplainableAF}, or a small, artificially-constructed corpus \cite{Wadden2020FactOF}. While some recent work explores verifying claims against a large-scale scientific corpus, it evaluates systems on their accuracy at predicting a single global truth label \cite{Stammbach2021TheCO}.

% TODO probably mention climate-fever?

\input{fig/teaser_wrapper.tex}

In this work, we aim to gain a better understanding of scientific claim verification against a large corpus, which we term \emph{open-domain scientific claim verification}. We are motivated by two research questions. First, are models trained to verify claims against a limited context (e.g. a small corpus) able to generalize to much larger corpora not seen during training, and can we reliably compare the generalization performance of different models in this setting? The ability to characterize model behavior under this kind of distribution shift is particularly important for scientific claim verification, since the body of scientific evidence is constantly expanding, as is the number of online corpora on which a fact verification system might be deployed. Second, does the open setting present novel NLP challenges that were less apparent in a more restricted context?

% TODO I'm here.

To make progress on these questions, we construct a new test set for open-domain scientific claim verification, which we call \scifactOpen. \scifactOpen builds on the \scifact dataset \cite{Wadden2020FactOF} (which we call \scifactOrig); it contains the same claims, and includes all evidence from \scifactOrig. In addition, we collect additional evidence from a corpus of 500K scientific research abstracts, using a \emph{pooling} strategy (popularized by the TREC competitions) to prioritize abstracts for human annotation. Pooling uses a collection of existing fact verification models to identify abstracts likely \support or \refute test set claims, and then collects human annotations for the candidate abstracts. The key decisions when collecting annotations via pooling are: (1) The choice of fact-checking models, (2) The criteria used to prioritize candidate abstracts for annotation, and (3) The number of candidates to annotate. We discuss these choices in depth in \S \ref{sec:data}, and perform experiments to confirm that the collected annotations are extensive enough to facilitate reliable model evaluation.

Using our newly-collected dataset, we find that generalization to the open-domain setting represents a substantial challenge for existing fact verification models, and that the best-performing model on \scifactOrig was over-fit to the abstracts in the original dataset. In addition, we find that conflicting evidence is fairly common in \scifactOpen, and is often caused by claim ambiguity: cases where one special case of the input claim is supported by evidence is refuted, and a different special case is refuted. We are optimistic that our new dataset, analysis, and suggested ``best practices'' for studying open-domain scientific claim verification will motivate future work on this relevant and challenging task.


==> table/_old/annot_counts_by_model.tex <==
\begin{tabular}{p{0.3\linewidth}p{0.2\linewidth}p{0.2\linewidth}p{0.1\linewidth}}
\toprule
{} &  \% Relevant &  \% Correct &  Total \\
Model          &              &             &        \\
\midrule
\sysnameTen    &         40.5 &        37.0 &    200 \\
\sysnameTwenty &         35.0 &        29.5 &    200 \\
\pjoint        &         45.5 &        41.0 &    200 \\
\vertserini    &         36.0 &        36.0 &    200 \\
\bottomrule
\end{tabular}


==> table/_old/annot_counts_by_num_systems.tex <==
\begin{tabular}{p{0.3\linewidth}p{0.2\linewidth}p{0.2\linewidth}p{0.1\linewidth}}
\toprule
\# Systems &  \% Relevant &  \% Correct &  Total \\
\midrule
         1 &         30.0 &        26.8 &    426 \\
         2 &         45.1 &        42.6 &    122 \\
         3 &         53.3 &        46.7 &     30 \\
         4 &         70.0 &        70.0 &     10 \\
\midrule
   Overall &         35.0 &        31.8 &    588 \\
\bottomrule
\end{tabular}



==> table/_old_annot_counts_wrapper.tex <==
\begin{table}[t]
  \footnotesize
  \centering

  \begin{subtable}{\linewidth}
    \input{table/_old_annot_counts_by_model.tex}
    \subcaption{Each row shows the accuracy of a particular model, on the top-200 predictions made by that model.}
    \label{tbl:annot_counts_by_system}
  \end{subtable}

  \begin{subtable}{\linewidth}
    \input{table/_old_annot_counts_by_num_systems.tex}
    \subcaption{The first row shows the overall accuracy on abstracts that a single system  identified as relevant. The second row shows accuracy on abstracts identified by two systems, etc. When multiple systems identify the same abstract as relevant, that abstract is more likely to contain evidence. \ib{what are relevance and correctness here? } Note that the overall total is 588 rather than 800 because multiple systems sometimes predict the same abstract.}
    \label{tbl:annot_counts_num_systems}
  \end{subtable}

  \caption{Accuracy of model predictions. ``\% Relevant'' indicates the percentage of abstracts containing relevant evidence. ``\% Correct'' indicates the percentage of correctly-labeled abstracts, where the label is chosen by majority vote over the four systems. ``Total'' indicates the total number of abstracts. \ib{ok, found the defintio of relevant and correct. Q: what conclusions you make from the numbers in the  ``Correct'' column?I don't feel like it is adding much but I could be missing something  }}
  \label{tbl:annot_counts}
\end{table}


==> table/_old_dataset_summary_scifact_orig.tex <==
\begin{table}[t]
    \footnotesize
    \centering
    \begin{tabular}{L{0.32\linewidth}L{0.28\linewidth}L{0.28\linewidth}}
        \toprule
                           & \scifactOrig & \scifactOpen \\
        \midrule
        Corpus size        & 5,183        & 500,000      \\
        Train + dev claims & 1,109        & -            \\
        Test claims        & 300          & 279          \\
        Test ECAPs         & 222          & 460          \\
        \bottomrule
    \end{tabular}

    \caption{Dataset summary. \dave{TODO change this and put it later; remove \scifactOrig}}
    \label{tbl:dataset_summary}
\end{table}


==> table/entity_overlap.tex <==
\begin{table}[t]
    \footnotesize
    \begin{tabular}{p{0.35\linewidth}p{0.1\linewidth}p{0.35\linewidth}}
        \toprule
        N shared entities & Count & \% relevant \\
        \midrule
        0                 & 131   & 16.8        \\
        1                 & 347   & 33.1        \\
        2                 & 168   & 39.9        \\
        3                 & 30    & 60.0        \\
        \bottomrule
    \end{tabular}
    \caption{Shows how frequently a predicted evidence abstract is relevant, as a function of how many entities it shares with the claim it's predicted to contain evidence for.}
\end{table}


==> table/error_analysis.tex <==
\begin{table}[t]
    \footnotesize

    \begin{subtable}{\linewidth}
        \centering
        \begin{tabular}{
                L{.19\linewidth}
                R{.15\linewidth}
                R{.14\linewidth}
                R{.17\linewidth}
                R{.1\linewidth}
            }
            \toprule
            \textbf{Error type} & Single sentence & Synonym & Hypo / hypernym & Other \\
            \cmidrule(lr){2-5}
            \textbf{Count}      & 8               & 6       & 4               & 2     \\
            \bottomrule
        \end{tabular}
        \caption{Errors where model missed an example..}
        \label{tbl:error_analysis_missed}
    \end{subtable}

    \begin{subtable}{\linewidth}
        \centering
        \begin{tabular}{
                L{.25\linewidth}
                L{.17\linewidth}
                L{.17\linewidth}
                L{.17\linewidth}
            }
            \toprule
            \textbf{Agreement}   & \textbf{Subject} & \textbf{Property} & \textbf{Context} \\
            \midrule
            \textbf{Matched}     & 16               & 12                & 10               \\
            \textbf{Mis-matched} & 3                & 5                 & 9                \\
            \textbf{Irrelevant}  & 1                & 3                 & 1                \\
            \bottomrule
        \end{tabular}
        \caption{Errors where model predicted an example.}
        \label{tbl:error_analysis_predicted}
    \end{subtable}

    \caption{
        Error analysis.
    }
    \label{tbl:error_analysis}
\end{table}


==> table/error_analysis_example.tex <==
\begin{table*}[t]
    \footnotesize
    \centering

    \begin{tabular}{
            L{.09\linewidth}
            R{.34\linewidth}
            R{.15\linewidth}
            R{.15\linewidth}
            R{.15\linewidth}
        }
        \toprule
                  & Text                                                                   & Subject         & Property              & Context              \\
        \midrule
        Claim     & Transmission of avian influenza between humans has not been observed.  & Avian influenza & Cannot be trasnmitted & Between humans       \\
        \cmidrule(lr){1-5}
        Abstract  & Transmission rates of avian influenza among bird species are very low. & Avian influenza & Has low transmission  & Between bird species \\
        \cmidrule(lr){1-5}
        Agreement &                                                                        & Match           & Mismatch              & Mismatch \\
        \bottomrule
    \end{tabular}

    \caption{
        Example error analysis.
    }
    \label{tbl:error_analysis_example}
\end{table*}


==> table/evidence_count_examples.tex <==
\begin{table}[t]
    \footnotesize
    \centering

    \begin{tabular}{
            p{0.7\linewidth} | p{0.2\linewidth}
        }
        \toprule
        \textbf{Claim}                                                                      & \textbf{N evidence docs} \\
        \midrule
        Serotonin receptors play a role in depression                                       & 12                       \\
        \cmidrule(lr){1-2}
        Gene expression can be highly variable across genetically identical cells.          & 8                        \\
        \cmidrule(lr){1-2}
        Mitochondria play a major role in calcium homeostasis.                              & 6                        \\
        \cmidrule(lr){1-2}
        Hypertension can be accurately diagnosed with ambulatory blood pressure monitoring. & 5                        \\
        \midrule
        The PDPN gene activates the C-type lectin receptor (CLEC-2).                        & 0                        \\
        \cmidrule(lr){1-2}
        Genetic deletion of JAM-A decreases gut permeability.                               & 0                        \\
        \cmidrule(lr){1-2}
        No strong relationship has been found with Pioglitazone use and pancreatic cancer.  & 0                        \\
        \cmidrule(lr){1-2}
        Inhibiting HDAC6 decreases survival of mice with ARID1A mutated tumors.             & 0                        \\
        \bottomrule
    \end{tabular}

    \caption{Examples of claims with lots of evidence, and no evidence. Claims with lots of evidence tend to discuss general entity types and / or highly-studied entities (e.g. Depression, mitochondria, hypertension), while claims with no evidence deal with very specific entity types (e.g. Jam-A, Pioglitazone, ARID1A)}
    \label{tbl:evidence_examples}
\end{table}


==> table/evidence_count_wrapper.tex <==
% No longer used; I split these out.

\begin{table}[t]
    \footnotesize
    \centering

    \input{table/claim_evidence_alloc.tex}
    \input{table/evidence_count_examples_short.tex}

    \caption{
        Properties of claims for which new evidence was discovered during pooled data collection, vs. claims with no new evidence. Well-studied ECAPs tend to be shorter and mention fewer entities. The entities which they do mention are more common, as measured by the number of results returned by a PubMed search.
        }
    \label{tbl:claim_evidence_analysis}
\end{table}


==> table/evidence_counts.tex <==
\begin{table}[t]
    \footnotesize
    \centering
    \begin{tabular}{lrrrrr}
        \toprule
                     & 0   & 1   & 2  & 3 & 4+ \\
        \midrule
        \scifactOrig & 89  & 175 & 13 & 1 & 1  \\
        \scifactOpen & 187 & 36  & 16 & 7 & 33 \\
        \bottomrule
    \end{tabular}
    \caption{
        Allocation of evidence across claims. In \scifactOrig, 175 / 271 claims have exactly one supporting or refuting document. In the newly-collected annotations, no new evidence was found for 187 claims, while 4 or more new relevant abstracts were found for 33 claims. \dave{Make this table more clear.}
    }
    \label{tbl:evidence_allocation}
\end{table}


==> table/metrics_include_self_true.tex <==
\begin{tabular}{
    L{0.35\linewidth}R{0.06\linewidth}R{0.06\linewidth}R{0.06\linewidth}R{0.06\linewidth}R{0.06\linewidth}
    }
    \toprule
    Model         & P    & R    & F1   & AP   & F1-Orig \\
    \midrule
    \vertserini   & 25.0 & 67.2 & 36.4 & 27.5 & 68.2    \\
    \pjoint       & 54.7 & 46.5 & 50.3 & 40.5 & 69.1    \\
    \sysname      & 73.6 & 40.7 & 52.4 & 44.9 & 72.5    \\
    \sysnameTen   & 49.6 & 53.0 & 51.3 & 43.4 & 67.6    \\
    \cmidrule(lr){1-6}
    \arsjoint$^*$ & 46.1 & 37.6 & 41.4 & -    & 68.1    \\
    \bottomrule
\end{tabular}


==> table/metrics_include_self_true_raw_less_studied.tex <==
\begin{tabular}{lrrrr}
    \toprule
    {}                 & P    & R    & F1   & average_precision \\
    model              &      &      &      &                   \\
    \midrule
    vert5erini         & 20.9 & 69.1 & 32.1 & 25.5              \\
    paragraph_joint    & 53.2 & 53.2 & 53.2 & 43.8              \\
    longformer_20_full & 72.7 & 58.4 & 64.8 & 56.9              \\
    longformer_10_full & 44.8 & 63.5 & 52.6 & 52.7              \\
    arsjoint           & 51.0 & 52.4 & 51.7 & 27.0              \\
    \bottomrule
\end{tabular}


==> table/metrics_include_self_true_raw_well_studied.tex <==
\begin{tabular}{lrrrr}
    \toprule
    {}                 & P    & R    & F1   & average_precision \\
    model              &      &      &      &                   \\
    \midrule
    vert5erini         & 31.7 & 65.2 & 42.7 & 30.0              \\
    paragraph_joint    & 57.0 & 39.6 & 46.8 & 40.1              \\
    longformer_20_full & 76.1 & 22.5 & 34.7 & 33.6              \\
    longformer_10_full & 59.3 & 42.3 & 49.4 & 38.6              \\
    arsjoint           & 37.5 & 22.5 & 28.1 & 11.3              \\
    \bottomrule
\end{tabular}


==> table/metrics_wide_omissions.tex <==
% Version of table with omitted metrics as well.

\begin{tabular}{
        L{0.16\linewidth}
        *{11}{P{0.045\linewidth}}
    }
    \toprule

                   & \multicolumn{3}{c}{\textbf{\scifactOrig}} & \multicolumn{4}{c}{\textbf{\scifactOpen} (Include self)} & \multicolumn{4}{c}{\textbf{\scifactOpen} (Omit self)} \\
    \cmidrule(lr){2-4} \cmidrule(lr) {5-8} \cmidrule(lr) {9-12}
    \textbf{Model} & P    & R    & F1                          & P    & R    & F1            & AP                         & P    & R    & F1            & AP                      \\
    \midrule
    \vertserini    & 64.0 & 73.0 & 68.2                        & 25.0 & 67.2 & 36.4          & 27.5                       & 19.9 & 65.3 & 30.5          & 17.3                    \\
    \pjoint        & 75.8 & 63.5 & 69.1                        & 54.7 & 46.5 & 50.3          & 40.5                       & 41.4 & 43.2 & 42.3          & 31.4                    \\
    \sysname       & 73.8 & 71.2 & \textbf{72.5}               & 73.6 & 40.7 & \textbf{52.4} & \textbf{44.9}              & 64.6 & 42.9 & \textbf{51.6} & \textbf{41.4}           \\
    \sysnameTen    & 63.0 & 73.0 & 67.6                        & 49.6 & 53.0 & 51.3          & 43.4                       & 38.8 & 50.0 & 43.7          & 36.0                    \\
    \cmidrule(lr){1-12}
    \arsjoint$^*$  & 72.2 & 70.3 & 71.2                        & -    & -    & -             & -                          & 46.1 & 37.6 & 41.4          & -                       \\
    \bottomrule
\end{tabular}


==> table/partial_evidence_complicated.tex <==
\begin{table}[t]
    \footnotesize
    \centering

    \begin{subtable}{\linewidth}
        \centering
        \begin{tabular}{
                L{.7\linewidth}
                R{.1\linewidth}
            }
            \toprule
            \textbf{Category}                               & \textbf{CAPs} \\
            \midrule
            \textbf{Evidence contains relevant information}           & 206 \\
            \cmidrule(lr){1-2}
            \hspace{3mm}Evidence matches claim              & 115           \\
            \hspace{3mm}Evidence more specific than claim   & 53            \\
            \hspace{3mm}Evidence more general than claim    & 18            \\
            \hspace{3mm}Evidence closely related to claim   & 20            \\
            \midrule
            \textbf{Evidence has no relevant information} & 110           \\
            \bottomrule
        \end{tabular}
        \caption{Specificity relationship between CAPS in the annotation pool. Mismatches are common, occurring in 44\% of cases where the abstract contains evidence relevant to claim.}
        \label{tbl:partial_evidence_counts_complicated}
    \end{subtable}


    \begin{subtable}{\linewidth}
        \begin{tabular}{
                L{0.95\linewidth}
            }
            \toprule
            \textbf{Claim}: Teaching hospitals provide better care than non-teaching hospitals.                                                                  \\
            \cmidrule(lr){1-1}
            \textbf{Evidence}: Teaching centers \dots prolong survival \emph{in women with any gynecological cancer} compared to community or general hospitals. \\
            \cmidrule(lr){1-1}
            \textbf{Revised claim}: Teaching hospitals provide better \emph{gynecological cancer} care than non-teaching hospitals                               \\
            \bottomrule
        \end{tabular}
        \caption{A CAP where the evidence \supports a special case of the claim, paired with a \emph{revised} version of the claim that matches the evidence. The claim discusses medical care overall, while the evidence discusses gynecological cancer care specifically.}
        \label{tbl:partial_evidence_example_complicated}
    \end{subtable}

    \caption{
        Claim / evidence specificity mismatch in \scifactOpen.
    }
    \label{tbl:partial_evidence}
\end{table}


==> table/partial_evidence_rules.tex <==
\begin{table}[t]
    \footnotesize
    \centering

    \begin{tabular}{
            L{0.60\linewidth} | R{0.30\linewidth}
        }
        \toprule
        \textbf{Relation}                     & \textbf{Label $y(c, a)$} \\
        \midrule
        $a$ \supports a \emph{special case} of $c$   & \supports                \\
        \cmidrule(lr){1-2}
        $a$ \supports a \emph{generalization} of $c$ & \nei                     \\
        \cmidrule(lr){1-2}
        $a$ \refutes a \emph{special case} of $c$    & \nei                     \\
        \cmidrule(lr){1-2}
        $a$ \refutes a \emph{generalization} of $c$  & \refutes                 \\
        \bottomrule
    \end{tabular}

    \caption{Rules for labeling ambiguous relationships between claim $c$ and abstract $a$.
    }
    \label{tbl:foo}
\end{table}


==> table/raw/evidence_counts_raw.tex <==
\begin{tabular}{lrrrrr}
\toprule
{} &    0 &    1 &   2 &  3 &  4+ \\
\midrule
Scifact-Orig &   89 &  175 &  13 &  1 &   1 \\
Scifact-Open &  187 &   36 &  16 &  7 &  33 \\
\bottomrule
\end{tabular}


==> table/raw/metrics_include_self_false_raw.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &    P &    R &   F1 &  average_precision \\
model              &      &      &      &                    \\
\midrule
arsjoint           & 46.1 & 37.6 & 41.4 &               18.0 \\
longformer_10_full & 45.7 & 51.1 & 48.3 &               41.2 \\
longformer_20_full & 72.4 & 42.4 & 53.5 &               44.2 \\
paragraph_joint    & 42.2 & 40.8 & 41.5 &               31.1 \\
vert5erini         & 20.8 & 63.0 & 31.2 &               17.5 \\
\bottomrule
\end{tabular}


==> table/raw/metrics_include_self_true_raw.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &    P &    R &   F1 &  average_precision \\
model              &      &      &      &                    \\
\midrule
arsjoint           & 46.1 & 37.6 & 41.4 &               18.0 \\
longformer_10_full & 49.6 & 53.0 & 51.3 &               43.4 \\
longformer_20_full & 73.6 & 40.7 & 52.4 &               44.9 \\
paragraph_joint    & 54.7 & 46.5 & 50.3 &               40.5 \\
vert5erini         & 25.0 & 67.2 & 36.4 &               27.5 \\
\bottomrule
\end{tabular}


==> table/raw/model_omission_full_raw.tex <==
\begin{tabular}{lllrrrr}
\toprule
{} &             model &  omitted &    P &    R &   F1 &   AP \\
\midrule
0 &        VerT5erini &    False & 25.0 & 67.2 & 36.4 & 27.5 \\
1 &        VerT5erini &     True & 19.9 & 65.3 & 30.5 & 17.3 \\
2 &    ParagraphJoint &    False & 54.7 & 46.5 & 50.3 & 40.5 \\
3 &    ParagraphJoint &     True & 41.4 & 43.2 & 42.3 & 31.4 \\
4 &         MultiVerS &    False & 73.6 & 40.7 & 52.4 & 44.9 \\
5 &         MultiVerS &     True & 64.6 & 42.9 & 51.6 & 41.4 \\
6 &  MultiVerS\$\_\{10\}\$ &    False & 49.6 & 53.0 & 51.3 & 43.4 \\
7 &  MultiVerS\$\_\{10\}\$ &     True & 38.8 & 50.0 & 43.7 & 36.0 \\
8 &          ARSJoint &    False & 46.1 & 37.6 & 41.4 & 18.0 \\
9 &          ARSJoint &     True & 45.3 & 39.2 & 42.0 & 18.3 \\
\bottomrule
\end{tabular}


==> table/raw/model_omission_raw.tex <==
\begin{tabular}{lrrr}
\toprule
{} &  Included &  Omitted &  Pct change \\
model            &           &          &             \\
\midrule
VerT5erini       &      36.4 &     30.5 &       -16.3 \\
ParagraphJoint   &      50.3 &     42.3 &       -15.9 \\
MultiVerS        &      52.4 &     51.6 &        -1.5 \\
MultiVerS\$\_\{10\}\$ &      51.3 &     43.7 &       -14.7 \\
ARSJoint         &      41.4 &     42.0 &         1.4 \\
\bottomrule
\end{tabular}


==> table/raw/mu_boot.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &    P &    R &   F1 &  average_precision \\
model              &      &      &      &                    \\
\midrule
vert5erini         & 25.1 & 67.2 & 36.5 &               28.0 \\
paragraph_joint    & 54.9 & 46.5 & 50.3 &               40.7 \\
longformer_20_full & 73.4 & 40.6 & 52.2 &               44.9 \\
longformer_10_full & 49.5 & 53.2 & 51.2 &               43.6 \\
arsjoint           & 46.2 & 37.7 & 41.4 &               18.1 \\
\bottomrule
\end{tabular}


==> table/raw/precision_by_n_systems_raw.tex <==
\begin{tabular}{lrrr}
\toprule
n\_systems &  total &  relevant &  pct\_relevant \\
\midrule
        1 &    528 &       154 &          29.2 \\
        2 &    150 &        71 &          47.3 \\
        3 &     44 &        20 &          45.5 \\
        4 &     10 &         6 &          60.0 \\
      all &    732 &       251 &          34.3 \\
\bottomrule
\end{tabular}


==> table/raw/sigma_boot.tex <==
\begin{tabular}{lrrrr}
    \toprule
    {}                 & P   & R   & F1  & average_precision \\
    model              &     &     &     &                   \\
    \midrule
    vert5erini         & 1.9 & 2.9 & 2.2 & 3.2               \\
    paragraph_joint    & 3.2 & 3.5 & 2.7 & 3.1               \\
    longformer_20_full & 2.9 & 3.3 & 3.0 & 3.7               \\
    longformer_10_full & 3.0 & 3.7 & 2.4 & 3.4               \\
    arsjoint           & 2.9 & 3.4 & 2.7 & 2.2               \\
    \bottomrule
\end{tabular}

